UrbanFly: Uncertainty-Aware Planning for Navigation Amongst High-Rises with Monocular Visual-Inertial SLAM Maps

We present UrbanFly: an uncertainty-aware real-time planning framework for quadrotor navigation in urban high-rise environments. A core aspect of UrbanFly is its ability to robustly plan directly on the sparse point clouds generated by a Monocular Visual Inertial SLAM (VINS) backend. It achieves this by using the sparse point clouds to build an uncertainty-integrated cuboid representation of the environment through a data-driven monocular plane segmentation network. Our chosen world model provides faster distance queries than the more common voxel-grid representation, and UrbanFly leverages this capability in two different ways leading to two trajectory optimizers. The first optimizer uses a gradient-free cross-entropy method to compute trajectories that minimize collision probability and smoothness cost. Our second optimizer is a simplified version of the first and uses a sequential convex programming optimizer initialized based on probabilistic safety estimates on a set of randomly drawn trajectories. Both our trajectory optimizers are made computationally tractable and independent of the nature of underlying uncertainty by embedding the distribution of collision violations in Reproducing Kernel Hilbert Space. Empowered by the algorithmic innovation, UrbanFly outperforms competing baselines in metrics such as collision rate, trajectory length, etc., on a high-fidelity AirSim simulator augmented with synthetic and real-world dataset scenes.

==> Algorithmic_results.tex <==
\section{Main Algorithmic Results}

\subsection{Collision Querying}

% As previously mentioned we consider the error in estimation of the size and orientation of the cuboids.  We draw $\mathbf{m}$ and $\mathbf{n}$ samples from the black-box error distribution of the yaw and size uncertainty.

The distance to collision of a query point $\mathbf{Q}$ is checked by querying the analytical SDF function of the cuboid that is given by Eq. ~\ref{box_sdf}. The result $d_{i}^{j}$ represents the distance  measured to a cube using the $i^{th}$ sample from the yaw angle distribution and the $j^{th}$ sample ($s^{j}$) from the size distribution and $|.|$ is the absolute value function.

\begin{equation}\label{box_sdf}
    d_{i}^{j} = \norm{ \max \Big(   \big(  \lvert T_{i}Q \rvert - s^{j} \big) , 0_{3 \times 1}  \Big)}_{2}
\end{equation}

 $T_{i}$ is a matrix defined by  Eq. ~\ref{transform1} and ~\ref{transform2} that transforms the query point $\mathbf{Q}$ from the world frame to the local coordinates of the cuboid, and $P_{org}$ is the origin of the cuboid in world frame. 

\noindent\begin{minipage}{.5\linewidth}
\begin{equation} \label{transform1}
  T_{i} =  \left[  \begin{array}{c|c}
R_{i}^{T} & -R_{i}^{T}P_{org} \\
\hline
0_{1 \times 3 } & 1
\end{array}\right]
\end{equation}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\vspace{-3mm}
\begin{equation} \label{transform2}
  R_{i}^{T} =  \begin{bmatrix}
\cos \psi_{i} & -\sin \psi_{i} & 0\\
\sin \psi_{i} & \cos \psi_{i} & 0\\
0 & 0 & 1 \\ 
\end{bmatrix}
\end{equation}
\end{minipage}


We draw $\mathbf{m}$ and $\mathbf{n}$ samples from the black-box error distribution of the yaw and size uncertainty, this leads to a total of $\mathbf{m} \times \mathbf{n}$ distance measurements. 




\subsection{Distribution over Constraint Violations}
During flight in uncertain environments despite maintaining a safe distance from the obstacle it might loose the fine features from the buildings. However, if we formulate a very conservative approach and move farther away from the buildings we loose the coarse features that are present at the boundaries of the building. Therefore there is a need to  maintain an optimal distance from the buildings such that the features are tracked.  We handle this requirement as follows 

Let $p_{f}$ represent the probability distribution of the distances of $f(d)$ i.e $p_{f}=  P(f(d))$, we transform this to a constrain violation function given by Eq. ~\ref{const_violation}, the resulting probability distribution is given denoted as $p_{\overline{f}}$. 

\begin{equation} \label{const_violation}
    \overline{f} = \max ( d_{i}^{j} - r_{max} , 0) + \max( r_{min} - d_{i}^{j} , 0)  
\end{equation}

Although computing the exact analytical shape of the distribution $p_{\overline{f}}$ is intractable we can make the following remarks about its shape.

\newtheorem{remark}{Remark}
\begin{remark} \label{des_dirac}
The best possible shape of $p_{\overline{f}}$ is given by a Dirac Delta distribution $p_{\delta}$ . In other words, $p_{\delta}$ acts as the desired distribution for $p_{\overline{f}}$  
\end{remark}
\begin{remark}\label{dirac_sim}
As $p_{\overline{f}}$ becomes increasingly similar to $p_{\delta}$, the probability that the UAV is at-least $r_{min}$ away from the obstacle an at-most $r_{max}$ away from the obstacle increases.
\end{remark}

The desired distribution is always fixed and well known as described in Remark ~\ref{des_dirac}. Remark \ref{dirac_sim} forms the the basis of our proposed reformulation of CCO to Eq. ~\ref{dist_matching_proposed}.

\begin{equation}
    \min_{\textbf{c}_x, \textbf{c}_y, \textbf{c}_z} l(\textbf{c}_x, \textbf{c}_y, \textbf{c}_z)+w l_{dist}(p_{\overline{f}}, p_{\delta})
    \label{dist_matching_proposed}
\vspace{-2mm}
\end{equation}

\subsection{Maximum Mean Discrepancy and Sample Approximation} 

The \textit{Maximum Mean Discrepancy} is a popular approach to quantify the similarity between two distributions in Reproducing Kernel Hilbert Space (RKHS) using sample level information. To this end, let $\mu_{p_{\overline{f}}}$ and $\mu_{p_{\delta}}$ represent the RKHS embedding of $p_{\overline{f}}$ and $p_{\delta}$ computed in the following manner.


\noindent\begin{minipage}{.5\linewidth}
\vspace{-3mm}
\begin{equation}
 \small
\mu_{p_{\overline{f} }} = \sum_{p=1}^n \sum_{q=1}^m \alpha_p \beta_q k(\overline{f_c}(d_p^q) , \cdot ) \label{kernel_mean_fover}
\end{equation}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\vspace{-3mm}
\begin{equation}
\mu_{p_{\delta}} =\sum_{p=1}^n \sum_{q=1}^m \alpha_p \beta_q k( 0 , \cdot ) \label{kernel_mean_dirac}
\end{equation}
\end{minipage}

where $d_{p}^{q}$ represents the distance measurement to a the $c^{th}$ cuboid with size sample $s_{p}$ and orientation $\psi_{q}$, for a given $\mathbf{(c_x, c_y, c_z, t)}$.  Please Note that $\mu_{\delta}$ represents the Dirac function (desired distribution) and the samples from it are all zeros.  Using Eq.  ~\ref{kernel_mean_fover} and ~\ref{kernel_mean_dirac} we can formulate the distance matching function ($\mathit{l_{dist}}$) as given in Eq. ~\ref{mmd_ldist}. 

\begin{equation}
\small    l_{dist} = \left\Vert \mu_{p_{\overline{f}}} - \mu_{p_{\delta}} \right \Vert_{2}^{2}
    \label{mmd_ldist}
\vspace{-1mm}
\end{equation}

It is worth re-iterating the point that MMD is a function of the trajectory coefficients and time $\mathbf{(c_x, c_y, c_z, t)}$ and the objective of the optimization problem is to arrive at the appropriate trajectory coefficients that would lead to minimization of MMD (i.e the distance distribution should match the dirac function) and the primary cost function given in Eq. ~\ref{dist_matching_proposed}.  We perform optimization using \textit{Cross Entropy Minimization} \cite{CEM1} \cite{iCEM} and is discussed in secion \ref{Traj_Optim}.


 
  
\subsection{Computing MMD}


Let ${s_{1}}, s_{2}, s_{3} , ..., s_{n}$ be the $\mathbf{n}$ samples from the size of the cuboid and let $\psi_{1} , \psi_{2} , .., \psi_{m}$ be the $\mathbf{m}$ samples from the orientation of the cuboid, sampled at a time step $\mathbf{t}$ for a given $(c_x, c_y, c_z)$. For the given distance measurements we map them to the samples of $p_{\overline{f}}$ constraint violation function given in Eq. ~\ref{const_violation}. In this section we derive the matrix representation of MMD.
We first expand Eq. ~\ref{mmd_ldist} as follows 

\vspace{-1.5mm}
\begin{align} 
\small
    \lVert \mu_{p_{\overline{f}}} -  \mu_{p_{\delta}} \lVert ^{2} = & \langle {\mu_{p_{\overline{f}}}(d)} , {\mu_{p_{\overline{f}}}(d)} \rangle - 2 \langle {\mu_{p_{\overline{f}} }}, {\mu_{p_{\delta}}} \rangle + \nonumber \\ & \langle {\mu_{p_{\delta}}} , {\mu_{p_{\delta}}} \rangle
\label{MMD_expand}
\vspace{-2mm}
\end{align}

substituting the kernel mean functions \ref{kernel_mean_fover} and \ref{kernel_mean_dirac} in \ref{MMD_expand} we obtain 

\begin{subequations} \label{kernel_trick}
\small
\begin{gather} 
    \langle \mu_{p_{\overline{f}}}(d), \mu_{p_{\overline{f}}} \rangle = 
    \langle \sum_{p=1}^n \sum_{q=1}^m \alpha_p \beta_q k(\overline{f}(d_p^q) , \cdot ) , \sum_{p=1}^n \sum_{q=1}^m \alpha_p \beta_q k(\bar{f}(d_p^q)) \rangle \\
\langle \mu_{p_{\bar{f}}}, \mu_{p_{\delta}} \rangle = \langle \sum_{p=1}^n \sum_{q=1}^m \alpha_p \beta_q k (\bar{f} (d_p^q), \cdot), \sum_{p=1}^n \sum_{q=1}^m \lambda_p \varphi_q k (0, \cdot) \rangle \\ 
\langle \mu_{p_{\delta}}, \mu_{p_{\delta}} \rangle = 
\langle \sum_{p=1}^n \sum_{q=1}^m \lambda_{p} \varphi_{q} k (0, \cdot), \sum_{p=1}^n \sum_{q=1}^m \lambda_p \varphi_q k (0, \cdot) \rangle
\end{gather}
\end{subequations}

Using the kernel trick Eq. \ref{kernel_trick} can be expressed in matrix form as given below 

%% Equation 4
\begin{align}
    \lVert \mu_{p_{\overline{f}}} - \mu_{p_{\delta}} \lVert ^2 = &
    C_{\alpha \beta} K_{\overline{f}\overline{f}} C_{\alpha \beta}^T - 2C_{\alpha\beta} K_{\overline{f}\delta}C_{\lambda\varphi}^T + \nonumber \\ & C_{\lambda\varphi} K_{\delta\delta} C_{\lambda\varphi}^T 
\end{align}


where $C_{\alpha \beta}$ and $C_{\lambda\varphi}$ are the weight vectors that are given by 

%% Equation 5
\begin{align*}
K_{\overline{f}\overline{f}} = \begin{bmatrix}
K^{00} & K^{01} & \dots & K^{0n}  \\
K^{10} & K^{11} & \dots & K^{1n}  \\
\vdots & \vdots & \ddots & \vdots \\
K^{m0} & K^{m1} & \dots & K^{mn}  \\
\end{bmatrix}
\end{align*}

%% Equation 6
\begin{align*}
K^{ab} = \begin{bmatrix}
k(d_a^0,d_b^0) & k(d_a^1, d_b^0) & \dots & k(d_a^m, d_b^0) \\
k(d_a^0,d_b^1) & k(d_a^1, d_b^0) & \dots & k(d_a^m, d_b^1) \\
\vdots & \vdots & \ddots & \vdots \\
k(d_a^0,d_b^n) & k(d_a^1, d_b^n) & \dots & k(d_a^m, d_b^n) \\
\end{bmatrix}
\end{align*}

\begin{align*}
K_{\bar{f}\delta} = \begin{bmatrix}
K_{\delta}^{00} & K_{\delta}^{01} & \dots & K_{\delta}^{0n}  \\
K_{\delta}^{10} & K_{\delta}^{11} & \dots & K_{\delta}^{1n}  \\
\vdots & \vdots & \ddots & \vdots \\
K_{\delta}^{m0} & K_{\delta}^{m1} & \dots & K_{\delta}^{mn}  \\
\end{bmatrix}
\end{align*}

%% Equation 6
\begin{align*}
K_{\delta}^{ab} = \begin{bmatrix}
k(d_a^0,0) & k(d_a^1, 0) & \dots & k(d_a^m, 0) \\
k(d_a^0,d_b^1) & k(d_a^1, d_b^0) & \dots & k(d_a^m, 0) \\
\vdots & \vdots & \ddots & \vdots \\
k(d_a^0,d_b^n) & k(d_a^1, d_b^n) & \dots & k(d_a^m, 0) \\
\end{bmatrix}
\end{align*}

\[ K_{\delta\delta} = \mathbf{1} \vspace{-2mm}\]


==> CEM.tex <==
\section{ Uncertainty Aware Motion Planning }


\[ \epsilon =  \{ \epsilon_{0} , \epsilon_{1} , \epsilon_{2} , ... , \epsilon_{n} \} \]

\[ T_{i} = \left[
\begin{array}{c|c}
R_{i}^{T} & -R_{i}^{T}P_{org} \\
\hline
0_{1 \times 3 } & 1
\end{array}
\right] \]

\begin{equation}
    d_{i}^{j} = \norm{ \max \Big(   \big(  \lvert T_{i}Q \rvert - S^{j} \big) , 0_{3 \times 1}  \Big)}_{2}
\end{equation}


\vspace{-2mm}
\begin{align}
    \overline{f} = \max(0, f(d(\textbf{c}_x, \textbf{c}_y, \textbf{c}_z, t)))
    \label{const_viol_function}
\vspace{-3mm}
\end{align}

\noindent\begin{minipage}{.5\linewidth}
\vspace{-3mm}
\begin{equation}
 \small
\mu_{p_{\overline{f} }} =\sum_{i=0}^{N} \sum_{j=0}^{M} \alpha_{i} \beta_{j} k( \overline{f}(d_{i}^{j} ), \cdot) \label{kernel_mean_fover}
\end{equation}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\vspace{-3mm}
\begin{equation}
\mu_{p_{\delta}} = \sum_{i=0}^{N} \sum_{j=0}^{M} \lambda_{i}\Psi_{j} k(0,  \cdot) \label{kernel_mean_dirac}
\end{equation}
\end{minipage}

\begin{equation}
\small    l_{dist} = \left\Vert \mu_{p_{\overline{f}}} - \mu_{p_{\delta}} \right \Vert_{2}^{2}
    \label{mmd_ldist}
\end{equation}


\begin{align} 
\small
    \lVert \mu_{p_{\overline{f}}} -  \mu_{p_{\delta}} \lVert ^{2} = & \langle {\mu_{p_{\overline{f}}}(d)} , {\mu_{p_{\overline{f}}}(d)} \rangle - 2 \langle {\mu_{p_{\overline{f}} }}, {\mu_{p_{\delta}}} \rangle + \nonumber \\ & \langle {\mu_{p_{\delta}}} , {\mu_{p_{\delta}}} \rangle
\label{MMD_expand}
\vspace{-2mm}
\end{align}





==> Method.tex <==
\section{Problem Formulation}

\textbf{Assumption} We propose a trajectory planning framework that can navigate amongst skyscrapers. We assume that the buildings are planar and feature rich. We further, expect a reliable state-estimate from the VINS system, but we acknowledge the uncertainty in the estimated 3D planes obtained from the triangulated point clouds of the monocular VINS. 

The error in the cuboid estimation can be modelled considering the uncertainty in its size and orientation. The error distribution in the size in the form of $s_{i} = s + \epsilon_{i}$ where $s_{i} \in R^{3}$ consists of the length, breadth and height of the cuboid. The error in orientation is formulated as a distribution in the yaw, 
the angular error is in the form of $\psi_{i} = \psi + \eta_{i}$, for practical reasons we assume that the building cannot pitch or roll. $\epsilon_{i}$ and $\eta_{i}$ are samples drawn from a non-parametric distributions shown in figure \ref{fig:error_distros}.

\textbf{Monocular 3D Reconstruction}
We employ a popular monocular VINS described in \cite{vins_mono} to compute the odometry and a sparse point cloud of triangulated key points. We then use PlaneRCNN \cite{planercnn}, a data driven network, to generate the 2D plane segment masks from the RGB image. 
PlaneRCNN computes plane segment masks in the image, 3D plane parameters and pixel-wise depth map. We discard these plane parameters and depth map estimated by the network, as they are found to be unreliable in outdoor settings due to ledges and balconies on high-rise facades. Each triangulated 3D key point in the point cloud is then associated with a plane, if corresponding 2D key point observation falls within a plane segment mask in the image. The parameters $(a, b, c, d)$ of each plane are estimated using RANSAC.

Note that the uncertainty of the estimated plane parameters depends on accuracy of triangulated key points, which are effected by other variables viz., number of detected features, pose-estimate from visual-inertial system and area of detected plane masks.

We therefore, bound the uncertain 3D plane segments with a cuboid. In the rest of the paper we represent the obstacles as cuboids.

\textbf{Uncertainty in Mapping}
Our experiments confirm that the error in estimated normal and offset distributions are non-parametric \ref{fig:error_distros}.

The posterior distribution of the uncertain plane parameters in a bayesian framework can then be expressed as

\begin{equation}
    P(\mathbf{x}/\mathbf{\hat{x}}) = \frac{P(\mathbf{\hat{x}}/\mathbf{x})P(\mathbf{x})}{P(\mathbf{\hat{x})}}
\end{equation}

where $P(\mathbf{\hat{x}})$ represents the probability of the estimated parameter, which is a constant. $P(\mathbf{x})$ is a uniform prior probability distribution of occurrence. $P(\mathbf{\hat{x}}/\mathbf{x})$ is the likelihood of the estimated value, given a ground truth or true value obtained from our experiments in synthetic scene.

The posterior estimate is used to draw samples from the plane parameter error distribution. Then, we fit cuboids that bound 80\% of the uncertain planes, as shown in figure \ref{}. Each cuboid is bounded by six planes. These planes are used to compute the analytical planarity constraint 

\begin{equation}
    \label{eq:plane_constraint}
    \mathbf{n}_j^T.\mathbf{x}_i+d_j
\end{equation}

Based on the sign of the value of the constraint (\ref{eq:plane_constraint}), each plane divides a 3D space into two halfs viz., positive and negative half-spaces. The normals of the planes are defined such that they point towards the camera origin. So, the space outside a cuboid is the union of positive half-spaces of all 6 planes defined by the cuboid's faces. Similarity, the space inside the cuboid is an intersection of negative half-spaces of all 6 planes defined by the cuboid faces.

So, to avoid collisions, the waypoints should be in the positive half-space of all cuboids in the scene. However, due to uncertainty in the estimated plane parameters, the plane collision cost defined by \ref{eq:plane_constraint} cannot be directly used. Therefore, we compute the MMD cost defined in section IV-D.

\textbf{Trajectory Parameterization} We define a trajectory in two forms, namely, polynomial parameterization and way-point parameterization. The \textit{Polynomial Parameterization} is used by \textit{Planner-C} and is defined in the following manner:

\vspace{-1mm}
\begin{equation}
\small
\begin{bmatrix}
x(t_1)\\
x(t_2)\\
\dots\\
x(t_n)
\end{bmatrix} = \textbf{P}\textbf{c}_{x}, \begin{bmatrix}
\dot{x}(t_1)\\
\dot{x}(t_2)\\
\dots\\
\dot{x}(t_n)
\end{bmatrix} = \dot{\textbf{P}}\textbf{c}_{x}, \begin{bmatrix}
\ddot{x}(t_1)\\
\ddot{x}(t_2)\\
\dots\\
\ddot{x}(t_n)
\end{bmatrix} = \ddot{\textbf{P}}\textbf{c}_{x}.
\label{param}
\vspace{-1mm}
\end{equation}

\noindent where, $\textbf{P}, \dot{\textbf{P}}, \ddot{\textbf{P}}$ are matrices formed with time-dependent basis functions (e.g polynomials) and $\textbf{c}_{x}$ are the coefficients associated with the basis functions. Similar expressions can be written for $y(t), z(t)$ as well in terms of coefficients $\textbf{c}_y, \textbf{c}_z$, respectively. \\  

\cite{STOMP} Proposes the way-point parameterization of the trajectory, it consists of $\mathbf{K}$ noisy trajectories in the form of $ \Tilde{\theta_{0}} ,  \Tilde{\theta_{1}} , ....,  \Tilde{\theta_{k}}$ with way-points as the parameters $\Tilde{\theta_{i}} = \Tilde{\theta} + \epsilon_{i} $ and $\epsilon_{i} \in \mathcal{N}(0, R^{-1})$ where $\mathcal{N}$ is a normal distribution with 0 mean and $R^{-1}$ is the inverse of the finite difference matrix which is used as the covariance of the normal distribution. \textit{Planner-S} uses the way-point parameterization


\textbf{Optimal Motion Planning } \noindent For an environment with $\mathbf{C}$ cuboids, our cost function (\ref{cost}) encourages safe and smooth trajectory by mapping the trajectory coefficients to penalties on higher-order motion derivatives such as jerk and penalising the violation of acceleration and velocity limit. 

\vspace{-4mm}
\begin{subequations}
   \begin{align}
       \min l(\textbf{c}_x, \textbf{c}_y, \textbf{c}_z) \label{cost} \\
        P( f_{c}(d) \leq  0 ) \geq \eta, \forall t, s, \psi , c \label{chance_const}
   \end{align}
\vspace{-2mm}
\end{subequations}
\vspace{-0.6cm}
\begin{align}
    f_{c}(d) = r_{safe}- d_{c}(\textbf{c}_x, \textbf{c}_y, \textbf{c}_z, t , s_{i}, \psi  ) \forall c \in [1, C]
    \label{const_func}
\vspace{-4mm}
\end{align}


 The function $d(.)$ maps the coefficients to the distance to the $c^{th}$ cuboid, with size $s_{i}$, orientation $\psi_{i}$ at time $t$. Furthermore, the chance constrain (\ref{chance_const}) ensures that the probability of the distance to the cube being less than $r_{safe}$ is above a specified threshold $\eta$. Constrains in the form of (\ref{chance_const}) are generally computationally intractable. Thus to make formulation a computational possibility, previous works \cite{rkhs_ral} \cite{boyd_chance} tend to make two common assumption, firstly the obstacles are bounded in geometric shapes such as cuboids or ellipsoids and an analytical function is used to query the distance, secondly the underlying uncertainty is assumed to be a Gaussian. In this work we relax the second assumption, and acknowledge that the uncertainty is non-parametric. 
 
 \textbf{Reformulation of Safe Trajectory planning as a distribution matching problem}  
 From our previous work \cite{rkhs_ral} [yet to be written ] 
 


==> equations.tex <==
%% Equation 1, 2, 3
\begin{subequations}
\small
\begin{gather} 
    \langle \mu_{p_{\overline{f}}}(d), \mu_{p_{\overline{f}}} \rangle = 
    \langle \sum_{p=1}^n \sum_{q=1}^m \alpha_p \beta_q k(\overline{f}(d_p^q) , \cdot ) , \sum_{p=1}^n \sum_{q=1}^m \alpha_p \beta_q k(\bar{f}(d_p^q)) \rangle \\
\langle \mu_{p_{\bar{f}}}, \mu_{p_{\delta}} \rangle = \langle \sum_{p=1}^n \sum_{q=1}^m \alpha_p \beta_q k (\bar{f} (d_p^q), \cdot), \sum_{p=1}^n \sum_{q=1}^m \lambda_p \varphi_q k (0, \cdot) \rangle \\ 
\langle \mu_{p_{\delta}}, \mu_{p_{\delta}} \rangle = 
\langle \sum_{p=1}^n \sum_{q=1}^m \lambda_{p} \varphi_{q} k (0, \cdot), \sum_{p=1}^n \sum_{q=1}^m \lambda_p \varphi_q k (0, \cdot) \rangle
\end{gather}
\end{subequations}

%% Equation 4
\begin{align}
    \lVert \mu_{p_{\bar{f}}} - \mu_{p_{\delta}} \lVert ^2 = &
    C_{\alpha \beta} K_{\bar{f}\bar{f}} C_{\alpha \beta}^T - 2C_{\alpha\beta} K_{\bar{f}0}C_{\lambda\varphi}^T + \nonumber \\ & C_{\lambda\varphi} K_{00} C_{\lambda\varphi}^T 
\end{align}

%% Equation 5
\begin{align*}
K_{\bar{f}\bar{f}} = \begin{bmatrix}
K^{00} & K^{01} & \dots & K^{0n}  \\
K^{10} & K^{11} & \dots & K^{1n}  \\
\vdots & \vdots & \ddots & \vdots \\
K^{m0} & K^{m1} & \dots & K^{mn}  \\
\end{bmatrix}
\end{align*}

%% Equation 6
\begin{align*}
K^{ab} = \begin{bmatrix}
K(d_a^0,d_b^0) & K(d_a^1, d_b^0) & \dots & K(d_a^m, d_b^0) \\
K(d_a^0,d_b^1) & K(d_a^1, d_b^0) & \dots & K(d_a^m, d_b^1) \\
\vdots & \vdots & \ddots & \vdots \\
K(d_a^0,d_b^n) & K(d_a^1, d_b^n) & \dots & K(d_a^m, d_b^n) \\
\end{bmatrix}
\end{align*}



==> methodology.tex <==
In this section we present the components of our pipeline in detail. Before that, we give a brief overview of the pipeline in the following paragraph.

\subsubsection{Overview}
The RGB images captured from a monocular camera are pre-processed to extract key points. We then use Plane-RCNN \cite{planercnn}, a deep network to detect plane segment masks. Monocular visual-inertial odometry (VINS-Mono \cite{vins_mono}) then fuses the pre-integrated IMU measurements with estimated upto-scale poses from visual features. It also optimizes the computed poses using factor-graph and computes a sparse 3D map. We then cluster the point cloud using plane masks and fit a plane to each clustered point cloud using RANSAC to find the plane parameters and remove outlier points. 
We then generate collision-free trajectories considering the uncertainty in the reconstructed plane segments. Optimal trajectory that reduces the uncertainty is then used for navigation towards the goal point.

 
\subsubsection{Preprocessing}
We use PlaneRCNN \cite{planercnn}, a deep neural architecture to predict the plane segment masks in the RGB image. After getting the masks, we filter out the ground and the sky. We also remove masks which are less than 8000 pixels in area. 

\subsubsection{Monocular Visual-Inertial Odometry}
Although detailed description of VINS-Mono is beyond the scope of this paper, we briefly describe the steps involved in estimating the odometry from vision and IMU measurements.

The system starts with measurement preprocessing, in which planar features are extracted and tracked, and IMU measurements between two consecutive frames are preintegrated. The initialization procedure provides all necessary values, including, pose, velocity, gravity vector, gyroscope bias, and three-dimensional (3-D) feature location, for bootstrapping
the subsequent nonlinear optimization-based VIO.

We use the estimated camera pose to transfer the 3D planar features into the world frame. These features are used in the subsequent step for estimating the plane segment parameters.

\subsection{Mapping}
The map generated from the key points triangulated in the previous step is sparse and cannot be used for trajectory planning. We, therefore, cluster the 3D keypoints based on their 2D observations in the plane segment mask. For each cluster of 3D points, we fit a plane using RANSAC. Further, we fit a cuboid to the inlier points. This step is repeated as more planar features are observed. We maintain a global map of cuboids, to use them in the trajectory planning. The pipeline is shown in \ref{fig:pipeline}.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=0.85\textwidth]{images/vins_features.png}\\[0.05\linewidth]
        \includegraphics[width=0.85\textwidth]{images/plane_masks.png}
        \caption{}
        \label{fig:pipeline_features_masks}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\linewidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images/map_paths_stomp.png}
        \caption{}
        \label{fig:pipeline_map_paths}
    \end{subfigure}
    \caption{Pipeline}
    \label{fig:pipeline}
\end{figure}

RGB images from the camera, the IMU (Inertial Measurement Unit) readings are passed to the visual-inertial odometry (VIO) algorithm.
VIO can be briefly described as follows. Visual-Inertial odometry detects and tracks keypoints in the image. Pre-integrated IMU measurements are used to compute the odometry in a factor graph optimization framework. VIO also computes the 3D features by triangulation of their 2D observations within the sliding window.

In parallel to VIO, we also run PlaneRCNN to compute the plane segment masks from the RGB images.

All the triangulated features which are observed within a plane segment mask in the image, belong to a single plane in 3D. Each plane is characterised by its normal($\boldsymbol{n}$) and offset ($\boldsymbol{d}$). These parameters are found using RANSAC (RANdom SAmple Consensus). We then fit a cuboid that bounds all the inlier points.

However, as mentioned earlier, the triangulated 3D features have uncertainty and thereby the plane parameters derived from them are also prone to uncertainty. From our experimental results, the uncertainty of plane normal and offset are characterized by the distribution shown in the figures. This distribution is obtained by comparing the estimated plane parameters with their ground truth values obtained over many runs in different synthetic and real environments in the simulator.

Then, we fit cuboids that bound the uncertain plane segment. Each cuboid is bounded by six planes. These planes are used to compute the analytical planarity constraint 

\begin{equation}
    \label{eq:plane_constraint}
    \mathbf{n}_j^T.\mathbf{x}_i+d_j
\end{equation}

Based on the sign of the value of the constraint (\ref{eq:plane_constraint}), each plane divides a 3D space into two halfs viz., positive and negative half-spaces. The normals of the planes are defined such that they point towards the camera origin. So, the space outside a cuboid is the union of positive half-spaces of all 6 planes defined by the cuboid's faces. Similarity, the space inside the cuboid is an intersection of negative half-spaces of all 6 planes defined by the cuboid faces.

So, to avoid collisions, the waypoints should be in the positive half-space of all cuboids in the scene. However, due to uncertainty in the estimated plane parameters, the plane collision cost defined by \ref{eq:plane_constraint} cannot be directly used. Therefore, we compute the MMD cost defined in the next section.

\subsection{Uncertainty aware trajectory Planning}
We consider STOMP-based planner as the baseline and compare its performance against the proposed CEM-based planner.

\begin{figure}
\centering
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/ransac_normal_distro.png}
        % \subcaption{Collision-free initial trajectories}
        \label{fig:normal_error_distro}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/ransac_plane_offset_distro.png}
        % \subcaption{Collision-free optimized trajectories}
        \label{fig:offset_error_distro}
    \end{subfigure}
    \caption{Error distribution of normals and plane offsets}
    \label{fig:error_distros}
\end{figure}

\subsubsection{MMD cost}
MMD (Maximum Mean Discrepancy) cost is computed by sampling the normals and plane offsets from the distributions shown in figure \ref{fig:error_distros}

\subsubsection{STOMP-based trajectory planning}
STOMP (Stochastic Trajectory Optimization for Motion Planning) \cite{STOMP} generates multiple noisy end-to-end trajectories that explore the space around an initial trajectory. In the subsequent step, we choose the trajectory that has the least initial collision cost. We then optimize a cost function based on obstacle and smoothness cost using a quadratic program solver.

This involves two steps: (1) initialization and (2) optimization. These steps are illustrated in the figure \ref{fig:STOMP_illustration}.

\begin{figure}
\centering
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/collision_free_topview_init.png}
        \subcaption{Collision-free initial trajectories}
        \label{fig:init_stomp_trajectories}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/collision_free_topview_optimized.png}
        \subcaption{Collision-free optimized trajectories}
        \label{fig:optim_stomp_trajectories}
    \end{subfigure}
    \caption{STOMP trajectories illustration}
    \label{fig:STOMP_illustration}
\end{figure}

The initialization consists of generating noisy trajectories as given by STOMP formulation. Each trajectory is represented by its waypoints. STOMP involves, to explain intuitively, generating random accelerations and integrating them to compute waypoints. This results in random continuous trajectories.

The optimization of the initialized trajectory is done by using the plane-half space constraints (illustrated in Figure 4). The cost function is the sum of accelerations. As shown in the figure, this optimization step generates a smooth trajectory.


\subsubsection{CEM-based trajectory planning}

In this method, instead of using a quadratic program, we use Cross-Entropy Minimization to optimize a STOMP initialized trajectory. Unlike the baseline, STOMP trajectory is generated only to the local goal and used for CEM.

==> temp_draft.tex <==
The steps of our approach can be described as follows:

Our goal is to navigate an aerial vehicle equipped with a single camera and an IMU to navigate to a goal point in outdoor urban environments.
Outdoor urban environments are densely populated with structures like skyscrapers and buildings. It is challenging due to various factors like texture less areas, inaccurate GPS, etc., Therefore we model the building facades as planes.

RGB images from the camera, the IMU (Inertial Measurement Unit) readings are passed to the visual-inertial odometry (VIO) algorithm.
VIO can be briefly described as follows. Visual-Inertial odometry detects and tracks keypoints in the image. Pre-integrated IMU measurements are used to compute the odometry in a factor graph optimization framework. VIO also computes the 3D features by triangulation of their 2D observations within the sliding window.

In parallel to VIO, we also run PlaneRCNN to compute the plane segment masks from the RGB images.


All the triangulated features which are observed within a plane segment mask in the image, belong to a single plane in 3D. Each plane is characterised by its normal(\boldsymbol{n}) and offset (\boldsymbol{d}). These parameters are found using RANSAC (RANdom SAmple Consensus).
However, as mentioned earlier, the triangulated 3D features have uncertainty and thereby the plane parameters derived from them are also prone to uncertainty. From our experimental results, the uncertainty of plane normal and offset are characterized by the distribution shown in the figures. This distribution is obtained by comparing the estimated plane parameters with their ground truth values obtained over many runs in different synthetic and real environments in the simulator.

Then, we fit cuboids that bound the uncertain plane segment. Each cuboid is bounded by six planes. These planes are used to compute the analytical planarity constraint $\mathbf{n_j}^T.\mathbf{x_i}+d_j$. Based on the sign of the value of the constraint, each plane divides a 3D space into two halfs viz., positive and negative half-spaces.

The normals of the planes are defined such that they point towards the camera origin. So, the space outside a cuboid is the union of positive half-spaces of all 6 planes defined by the cuboid's faces. Similarity, the space inside the cuboid is an intersection of negative half-spaces of all 6 planes defined by the cuboid faces.

So, to avoid collisions, the waypoints should be in the positive half-space of all the planes in the scene.

%%%%%%%%%%%%%%%      OLD    %%%%%%%%%%%%%%%%%%%%%%%%%
OLD:-

title:
VINS-Nav: A novel pipeline for end-to-end navigation of drones in outdoor planar scenes

abstract:
VINS-Mono\cite{vins_mono} is a versatile and robust state-estimator. In this paper, for the first time, we leverage the structural regularity in the outdoor urban scenes to achieve trajectory planning in the presence of mapping uncertainty arising from a monocular visual-inertial sensing modality. We showcase the results in synthetic as well as real world scenes using high-fidelity simulator Airsim\cite{airsim}. We contribute (1) a pipeline that combines deep learning method with multi-view geometry to reconstruct planar facades and (2) a novel uncertainty aware trajectory planner attuned to planar scenes.

Recent developments in robotics have enabled the usage of UAVs for various applications like aerial surveying and inspection, package delivery, etc., However, navigation of UAVs in urban scenes pose various challenges for localization, mapping and path planning. UAVs (Unmanned Aerial Vehicles) are constrained in terms of payload capability, compute power and battery life. Other constraints that arise due to the existing sensing methods. LiDARs are heavy and demand power from the battery. Stereo and depth cameras are not suitable for long range. Multi view stereo methods are computationally intensive. In contrast, we use a single camera and an IMU which are light weight and consume less power compared to other methods.

In addition to that, navigation of UAVs in outdoor urban scenes populated with tall structures like buildings and skyscrapers  pose various problems. Inaccurate GPS data due to multi-path fading, lack of external markers used in indoor scenes, lack of ground plane visibility, texture less areas that lack visual features are some of the challenges for localization. Also, path planning in such environments should avoid failure of SLAM (Simultaneous Localization And Mapping) while considering the uncertainty in reconstructed planar map.

Due the above stated problems the uncertainty in the reconstructed map is high. This breaks existing deterministic planners, as shown in figure 1. Although, voxel-grid based planners exist, they are computationally intensive. In contrast, our planner considers the  uncertainty in the planar obstacles to generate collision-free trajectories, with less computation cost, as shown in figure 2.

Therefore, we propose a pipeline that leverages the inherent planar structure of the buildings for mapping and navigation of a UAV (Unmanned Aerial Vehicle) using monocular RGB images and IMU data. We combine various modules that use deep learning and 3D vision to obtain an online reconstruction of the skyline suitable for path planning.

The proposed method therefore, supports the mapping and planning for navigation of UAVs (Unmanned Aerial Vehicles) in outdoor planar environments using a single camera and an IMU (Inertial Measurement Unit). Main components of our method are pre-processing of the RGB images, planar reconstruction using visual-inertial odometry and path planning considering the uncertainty in the map. 

The paper is organized as follows. In section 2, we describe outline the components of our pipeline. Then we report the datasets, experiments and the obtained results in section 3. Finally, we conclude the paper in Section 4.

\begin{table}[]
\caption{Benchmark Comparison on \textit{Urban Scene} }
\centering  
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l c  rrr}  
\hline\hline                       % inserting double-line 
\\ [-2ex]
Method  
&  Computation & Smoothness & Success & Traversed Length \\ 
& Time(s) & ($m^2/s^5$) & \%  & (m)\\ [0.5ex]
\hline
\\ [-2ex]
&mean: $0.182$ & $10.82$ & $\mathbf{83.87}$   &mean: $150.214$ \\ [-1ex]
\raisebox{1.5ex}{Ours (Planner-C)} & std: $0.055$ &   & & std:$16.304$   \\[1.0ex]
&mean: $\mathbf{0.036}$ & $20.85$ & $80.47$   &mean: $133.82$  \\ [-1ex]
\raisebox{1.5ex}{Ours (Planner -S)} & std: $0.026$ &   & & std:$21.53$   \\[1.0ex]
&mean: $0.077$ & $ 12.54$ & $18.42$  &mean: $46.44$ \\ [-1ex]
\raisebox{1.5ex}{CCO Voxel } & std: $0.001$ &   & & std:$1.37$ \\[0.5ex]
&mean: $0.086$ & $11.54$ & $46.66$ &mean: $47.44$  \\ [-1ex]
\raisebox{1.5ex}{CCO Voxel+PF+BV } & std: $0.001$ &   &  & std:$8.37$ \\[0.5ex]
% [1ex] adds vertical space
\hline                          % inserts single-line
\end{tabular}}
\label{table:benchmark_urban_scene}
\end{table}

\subsection{Path Length} Results in tables \ref{table:benchmark_synthetic}, \ref{table:benchmark_urban_scene} and figure \ref{fig:three_paths} validate the use of our planners for autonomous navigation over several hundred meters. Note that, the trajectory shown in the figure covers various scenarios viz., navigation in narrow streets between the buildings, over the road closer to the buildings and crossing an intersection, which is devoid of any structures like buildings. When the plane segments are beyond the detectable range, our method continues to execute the trajectory from the previous re-planning step. The trajectory is updated in the subsequent re-planning step once the structures become visible.

% ---------- some filler sentences -------------
We showcase the end-to-end navigation of an aerial vehicle in outdoor urban scenes, for the first time with a single camera and an IMU.

Due the above stated problems the uncertainty in the reconstructed is high. This breaks existing deterministic planners, as shown in figure 1. Although, voxel-grid based planners exist, they are computationally intensive. In contrast, we model the uncertainty in the planar obstacles to generate collision-free trajectories.

Trajectories from deterministic planners may lead to collisions. On the other hand, existing uncertainty aware planners rely on voxel-grid representation are computationally intensive. In contrast, our planner leverages the structural regularity in the scene to generate robust collision-free trajectories.

We, for the first time, leverage the structural regularity in the outdoor urban scenes to achieve trajectory planning in the presence of mapping uncertainty arising due to a single camera and an IMU system.

\captionsetup[subfloat]{labelformat=empty}
\begin{figure*}[h]%
    \centering
    \subfloat[Trial 1 ]{{\includegraphics[width=4cm]{images/Qualitative/Qualitative1.png} }}%
    \qquad
    \subfloat[Trial 2]{{\includegraphics[width=4cm]{images/Qualitative/Qualitative2.png} }}%
    \qquad
    \subfloat[Trial 3]{{\includegraphics[width=4cm, height =6.3cm]{images/Qualitative/Qualitative3.png} }}%
    \qquad
    \caption{ \footnotesize The qualitative demonstration of the working of \textit{UrbanFly CEM}, \textit{Trial 1} and \textit{Trial 2} depicts planning and execution of the trajectory in the \textit{Urban Scene 3D} environment, \textit{Trial 3} demonstrates the planning in the \textit{SquareStreet} environment. The figure on the top is the simulation environment and the reconstructed cuboids from the triangulated point cloud is shown below ( the distances given is the mean size of the plane), we can observe that in each of these cases the drone was able to travel long distances and avoid building like obstacles  }%
    \label{fig:Qualitative}%
    \vspace{-1.5em}
\end{figure*}

==> terminology.tex <==
\section{Method}
\subsection{Overview}
We propose a trajectory planning framework that enables the navigation of UAVs equipped with a single camera and an IMU amongst the skyscrapers. The RGB images captured from a monocular camera are pre-processed to extract key points. Monocular Visual-Inertial Odometry (VIO) \cite{vins_mono} estimates upto-scale poses from these key points. Then, metric poses are computed by fusing the upto-scale poses with pre-integrated IMU measurements . VIO also optimizes the computed poses using factor-graph and computes a sparse 3D map. We use Plane-RCNN \cite{planercnn}, a data driven network to detect plane segment masks. The sparse 3D map of triangulated points is clustered using the plane masks. Each triangulated 3D keypoint in the point cloud is then associated with a plane, if corresponding 2D key point observation falls within a plane segment mask in the image. We fit a plane to each cluster using RANSAC to find the plane parameters and remove outlier points. Following that, we describe the method of fitting a cuboid using the posterior distribution of the uncertain plane parameters in a bayesian framework. We then generate collision-free trajectories considering the uncertainty in the reconstructed plane segments. Optimal trajectory that reduces the uncertainty is then used for navigation towards the goal point.

We assume that the buildings are planar and feature rich. We further, expect a reliable state-estimate from the VINS system, but we acknowledge the uncertainty in the estimated 3D planes obtained from the triangulated point clouds of the monocular VINS.

\subsection{Terminology}
Before describing the components of our pipeline, we define the terms and their symbols used in this paper.

\subsubsection{3D plane representation}
A 3D plane is characterised as a 4-d vector ($\boldsymbol{n}$, $d$) or ($a, b, c, d$), where $\boldsymbol{n}$ is its unit normal$(a, b, c)$ and $d$ is the plane offset (defines the shortest distance from the origin).

Assuming a stable VINS initialization, we consider that the z-axis of global map coincides with the gravity vector. Further, we assume that the building facades are vertical. This constraints the plane normal to have uncertainty only in 1 DoF (degree-of-freedom) i.e., yaw, which is around the vertical axis in the global map.

Therefore, we characterize an uncertainty of the planes in their yaw (which effects the normal) and the plane offset.

\subsubsection{Cuboid representation}
As presented in the introduction, we bound the uncertain planes with a cuboid. A cuboid can be represented by its vertices (points), edges (line segments) or its faces (planes). As the method operates in a planar environment, we characterize a cuboid as a set of 6 planes in computing the collision cost.

\subsubsection{Trajectory Parameterization} We define a trajectory in two forms, namely, polynomial parameterization and way-point parameterization.

 \textit{Polynomial Parameterization} is used by \textit{Planner-C} and is defined in the following manner:

\vspace{-1mm}
\begin{equation}
\small
\begin{bmatrix}
x(t_1)\\
x(t_2)\\
\dots\\
x(t_n)
\end{bmatrix} = \textbf{P}\textbf{c}_{x}, \begin{bmatrix}
\dot{x}(t_1)\\
\dot{x}(t_2)\\
\dots\\
\dot{x}(t_n)
\end{bmatrix} = \dot{\textbf{P}}\textbf{c}_{x}, \begin{bmatrix}
\ddot{x}(t_1)\\
\ddot{x}(t_2)\\
\dots\\
\ddot{x}(t_n)
\end{bmatrix} = \ddot{\textbf{P}}\textbf{c}_{x}.
\label{param}
\vspace{-1mm}
\end{equation}

\noindent where, $\textbf{P}, \dot{\textbf{P}}, \ddot{\textbf{P}}$ are matrices formed with time-dependent basis functions (e.g polynomials) and $\textbf{c}_{x}$ are the coefficients associated with the basis functions. Similar expressions can be written for $y(t), z(t)$ as well in terms of coefficients $\textbf{c}_y, \textbf{c}_z$, respectively.

\textit{Way-point parameterization}, inspired by \cite{STOMP}, is used in \textit{Planner-S} in the following manner. It consists of $k$ noisy trajectories in the form of $ \Tilde{\theta_{0}} ,  \Tilde{\theta_{1}} , ....,  \Tilde{\theta_{k}}$ with way-points as the parameters $\Tilde{\theta_{i}} = \Tilde{\theta} + \epsilon_{i} $ and $\epsilon_{i} \in \mathcal{N}(0, R^{-1})$ where $\mathcal{N}$ is a normal distribution with 0 mean and $R^{-1}$ is the inverse of the finite difference matrix which is used as the covariance of the normal distribution.
